Document Understanding Dataset and Evaluation (DUDE)

We call on the Document AI (DocAI) community to reevaluate current methodologies and embrace the challenge of creating more practically-oriented benchmarks. Document Understanding Dataset and Evaluation (DUDE) seeks to remediate the halted research progress in understanding visually-rich documents (VRDs). We present a new dataset with novelties related to types of questions, answers, and document layouts based on multi-industry, multi-domain, and multi-page VRDs of various origins, and dates. Moreover, we are pushing the boundaries of current methods by creating multi-task and multi-domain evaluation setups that more accurately simulate real-world situations where powerful generalization and adaptation under low-resource settings are desired. DUDE aims to set a new standard as a more practical, long-standing benchmark for the community, and we hope that it will lead to future extensions and contributions that address real-world challenges. Finally, our work illustrates the importance of finding more efficient ways to model language, images, and layout in DocAI.

==> answer_grid.tex <==
\begin{table}
  \small
  \begin{tabular}{l l}
    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/stamp.pdf}}\vspace{1mm}\\}
      % \textbf{Stamp.}
      (E) What is the last date the document was received?\vspace{1mm}

      (A) What does the stamp indicate?
    \end{minipage}
    &
    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/signature.pdf}}\vspace{1mm}\\}
      % \textbf{Signature.}
      (E) Who signed the document?\vspace{1mm}

      (A) Is is easy to read individual letters in Kurts signature?
    \end{minipage}
    \vspace{5mm}
    \\

    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/symbol.pdf}}\vspace{1mm}\\}
      % \textbf{Symbol.}
      (E) What is the remark above the first staff?\vspace{1mm}

      (A) What's the type of clef in the piano part?
    \end{minipage}
    &
    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/table.pdf}}\vspace{1mm}\\}
      % \textbf{Table.}
      (E) Which sample has the accuracy 82\%?\vspace{1mm}

      (A) What's the difference between correctness \%s?
    \end{minipage}
    \vspace{5mm}
    \\

    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/figure.pdf}}\vspace{1mm}\\}
      % \textbf{Figure.}
      (E) What's the second largest component?\vspace{1mm}

      (A) Is the civil payroll cost larger than 50\%?
    \end{minipage}
    & 
    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/handwriting.pdf}}\vspace{1mm}\\}
      % \textbf{Handwriting.}
      (E) What is the time of incident?\vspace{1mm}

      (A) What's the time of the incident in 24-hour system?
    \end{minipage}
    \vspace{5mm}
    \\

    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/checkbox.pdf}}\vspace{1mm}\\}
      % \textbf{Checkbox.}
      (E) Is the company incorporated?\vspace{1mm}

      (A) Is the "No" checkbox in the section 3a checked?
    \end{minipage}
    &
    \begin{minipage}{.44\linewidth}
      {\centering\frame{\includegraphics[width=0.7\linewidth]{images/answer_grid/numerical.pdf}}\vspace{1mm}\\}
      % \textbf{Numerical.}
      (E) What has the largest price?\vspace{1mm}

      (A) What is the total price rounded to thousands?
    \end{minipage}
    % \vspace{5mm}
    % \\

    % \begin{minipage}{.45\linewidth}
    %   \centering
    %   \frame{\includegraphics[width=0.8\linewidth]{images/answer_grid/font.pdf}}
    %   % \textbf{Font style.}
    %   (E) What is the bolded text?\vspace{1mm}

    %   (A) What is the heading style, including the casing?
    % \end{minipage}
    % \vspace{5mm}
  \end{tabular}

  \caption{Questions with (E)xtractive and (A)bstractive answers for particular layout semantics under consideration. Note it is not an exhaustive list.}\label{tab:answer_grid}
\end{table}


==> document_grid.tex <==
\begin{figure}
\captionsetup[subfloat]{labelformat=empty}
\centering
\subfloat[application]{  \frame{\includegraphics[width=0.22\linewidth]{images/document_grid/application.pdf}}
}
\subfloat[certificate]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/certificate.pdf}}
}
\subfloat[diploma]{  \frame{\includegraphics[width=0.22\linewidth]{images/document_grid/diploma.pdf}}
}
\subfloat[e-mail]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/email.pdf}}
}
\hspace{0mm}
\subfloat[form]{   % ???
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/form.pdf}}
}
\subfloat[handwritten]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/handwritten.pdf}}
}
\subfloat[infographic]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/infographic.pdf}}
}
\subfloat[invoice]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/invoice.pdf}}
}
\hspace{0mm}
\subfloat[leaflet]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/leaflet.pdf}}
}
\subfloat[agreement]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/legal agreement.pdf}}
}
\subfloat[letter]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/letter.pdf}}
}
\subfloat[manual]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/manual.pdf}}
}
\hspace{0mm}
\subfloat[meeting]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/meeting detail.pdf}}
}
\subfloat[memo]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/memo.pdf}}
}
\subfloat[news]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/news article.pdf}}
}
\subfloat[order]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/order.pdf}}
}
\hspace{0mm}
\subfloat[poster]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/poster.pdf}}
}
\subfloat[presentation]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/presentation.pdf}}
}
\subfloat[report]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/report.pdf}}
}
\subfloat[request]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/request.pdf}}
}
\hspace{0mm}
\subfloat[resume]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/resume.pdf}}
}
\subfloat[sheet]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/sheet.pdf}}
}
\subfloat[specification]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/specification.pdf}}
}
\subfloat[ticket]{
\frame{\includegraphics[width=0.22\linewidth]{images/document_grid/ticket.pdf}}
}
% \subfloat[questionnaire]{
% \frame{\includegraphics[width=0.23\linewidth]{images/document_grid/questionnaire.pdf}}
% }
\caption{Excerpts from DUDE documents (one per type). Not an exhaustive list of document types collected.}
\label{fig:document_grid}
\end{figure}
